Communicating over the Torn-Paper Channel

We consider the problem of communicating over a channel that randomly "tears" the message block into small pieces of different sizes and shuffles them. For the binary torn-paper channel with block length $n$ and pieces of length ${\rm Geometric}(p_n)$, we characterize the capacity as $C = e^{-\alpha}$, where $\alpha = \lim_{n\to\infty} p_n \log n$. Our results show that the case of ${\rm Geometric}(p_n)$-length fragments and the case of deterministic length-$(1/p_n)$ fragments are qualitatively different and, surprisingly, the capacity of the former is larger. Intuitively, this is due to the fact that, in the random fragments case, large fragments are sometimes observed, which boosts the capacity.

==> Converse.tex <==
\begin{align}
nR &= H(W) \nonumber \\
&\leq I(W;\mathcal{Y})+n\epsilon_n \nonumber \\
&\leq I(X^n;\mathcal{Y})+n\epsilon_n \nonumber \\
&=H(\mathcal{Y})-H(\mathcal{Y}|X^n)+n\epsilon_n,
\end{align}
We analyze $H(\mathcal{Y})$ and $H(\mathcal{Y}|X^n)$ separately.
\begin{align}
H(\mathcal{Y}) \leq \sum_{i=1}^{K}{Y_i^{m_i}} \leq n.
\end{align}
Next, we have
\begin{align}
H(\mathcal{Y}|X^n) &= \underbrace{H(\mathcal{Y}|X^n,\vec{N},\vec{T})}_{~=~0} + I(\mathcal{Y};\vec{N},\vec{T}|X^n) \nonumber \\ 
&= I(\mathcal{Y};\vec{N},\vec{T}|X^n) \nonumber \\ 
&= H(\vec{N},\vec{T}|X^n)-H(\vec{N},\vec{T}|X^n,\mathcal{Y}), 
\end{align}

Processes $\vec{N}$ and $\vec{T}$ are independent from each other and from the signal. Thus,
\begin{align}
H(\vec{N},\vec{T}|X^n) = H(\vec{N},\vec{T}) = H(\vec{N}) + H(\vec{T}).
\end{align}
 
 As discussed in Section~\ref{Section:Problem}, the input sequence is chopped into segments whose lengths come from a Geometric$(p)$ process. More precisely, we will have $K-1$ independent segments and the last segment's length is $n - \sum_{j=1}^{K-1}{N_j}$. Thus, we have
 \begin{align}
 H(\vec{T}) = \sum_{k=1}^{n}{H(\vec{T}|K=k) \Pr(K=k)} = \sum_{k=1}^{n}{\log_2(k!) \Pr(K=k)},
 \end{align} 
 and in particular, as $n \rightarrow \infty$, we have $\Pr(K = np) \rightarrow 1$, and thus, 
 \begin{align}
 H(\vec{T}) \rightarrow \log_2\left( (np)! \right),
 \end{align}
 and using Stirling's approximation~\cite{}, we have
 \begin{align}
 H(\vec{T}) \approx (np) \log_2(np) \quad \text{as} \quad n \rightarrow \infty.
 \end{align}
 
On the other hand, for $H(\vec{N})$ we have 
\begin{align}
H(\vec{N}) = \underbrace{(np-1)}_{average~\#~of~segments} \times \underbrace{\frac{H(p)}{p}}_{=~Entropy~of~a~Geometric~RV} = nH(p).
\end{align} 
%{\color{blue} Last one, $N_K$, depends on others. So, the above entropy needs some revision.}
%{\color{red} OK, this is actually wrong, $K$ is a RV and has entropy. Needs to be calculated.}

Finally, we have {\color{blue} This needs more work.}
\begin{align}
H&(\vec{N}, \vec{T}|X^n,\mathcal{Y}) \nonumber \\
&= \underbrace{H(\vec{N}|X^n,\mathcal{Y})}_{=~0} + H(\vec{T}|X^n,\mathcal{Y},\vec{N}).
\end{align}
Again, as $n \rightarrow \infty$, we have $\Pr(K = np) \rightarrow 1$, and thus,
\begin{align}
H(\vec{T}|X^n,\mathcal{Y},\vec{N}) \rightarrow \frac{\sum_{k=1}^{np}{\log_2( k! ) \times 2^{\frac{n}{k}+1}}}{2^n}.
\end{align}
%and thus,
%\begin{align}
%\frac{1}{n} H(\vec{T}|X^n,\mathcal{Y},\vec{N}) \rightarrow 0.
%\end{align}

Putting these arguments back together, for large $n$, we have
\begin{align}
nR &= H(\mathcal{Y})-H(\mathcal{Y}|X^n)+n\epsilon_n \nonumber \\
&\leq n - (np) \log_2(np) - n H(p) + \frac{\sum_{k=1}^{np}{\log_2( k! ) \times 2^{\frac{n}{k}+1}}}{2^n} + n\epsilon_n.
\end{align}

\noindent \underline{\bf Observation:} As long as
\begin{align}
p \log_2(np) \rightarrow 0 ~\text{as}~ n \rightarrow \infty,
\end{align} 
the outer-bound is simply $1$.  

\noindent \underline{\bf Comparison to Ilan's work:} Ilan's paper is somewhat a subset of this result. In Ilan's paper, we have $n=m \beta \log(m)$ and fixed segment lengths $\beta \log(m)$. Setting $p = 1/(\beta \log(m))$ gives a worse channel than that paper which says capacity is $(1-1/\beta)$. What do we get?
\begin{align}
p \log_2(np) = \frac{1}{\beta}.
\end{align}
So, we recover that result.


==> converse04-12.tex <==
% !TEX root = main.tex


We consider a genie-aided approach to the converse, where encoder and decoder have knowledge of the tearing points $N_1,N_2,...$.
We will view the resulting channel as a set of parallel channels, each of which involves the fragments of roughly the same size.
More precisely, for a parameter $L$, we will let
% the $k$th channel will have input and output fragments given by
\al{
& \X_k = \left\{ \vX_i : \frac{k-1}{L} \log n \leq N_i < \frac{k}{L} \log n \right\}
\text{ and } \nonumber \\
& \Y_k = \left\{ \vY_i : \frac{k-1}{L} \log n \leq N_{T_i} < \frac{k}{L} \log n \right\},
}
for $k=1,2,...$,
and we will think of the transformation from $\X_k$ to $\Y_k$ as a separate channel.
Notice that the $k$th channel is intuitively similar to the shuffling channel with equal-length pieces considered in \cite{DNAStorageISIT}.
Also notice that 
\al{
E\left[|\Y_k|\right] & = E\left[ |\Y|\right] \Pr\left( \frac{k-1}{L} \log n \leq N_1 < \frac{k}{L} \log n \right) 
\nonumber \\
& = np \Pr\left( \frac{k-1}{L} \leq \frac{N_1}{\log n} < \frac{k}{L}  \right).
\label{eq:expyk}
}
Notice that, since $\lim_{n\to\infty} p_n \log n = \alpha$, $E\left[\frac{\alpha N_1}{\log n}\right] \to 1$ as $n \to \infty$.
Moreover, asymptotically, $\tilde N_1 = \frac{N_1}{\log n}$ approaches an ${\rm Exp}(\alpha)$ random variable.
This well known fact is stated as the following lemma.
\begin{lemma} \label{lem:exp1}
Let $F_{\alpha}(t) = e^{-\alpha t}$ be the complementary CDF of an ${\rm Exponential}(\alpha)$ random variable.
If $N^{(n)}$ is a ${\rm Geom}(p_n)$ random variable and $\lim_{n\to\infty} E[N^{(n)}]/\log n = \alpha$, then
\al{
\lim_{n\to \infty}
\Pr\left( N^{(n)} \geq \beta \log n \right) = F_\alpha(\beta).
}
\end{lemma}
Using Lemma~\ref{lem:exp1},
we have that 
\al{
\lim_{n\to \infty} \frac{E\left[|\Y_k|\right]}{np_n} 
& = \lim_{n\to\infty} \Pr\left( \frac{k-1}{L} \leq \frac{N_1}{\log n} < \frac{k}{L}  \right) \nonumber \\
& = e^{-\alpha (k-1)/L} - e^{-\alpha k/L}.
}
Moreover, using standard concentration inequalities, the probability that $|\Y_k|/(np_n)$ deviates significantly from $E|\Y_k|/(np_n)$ vanishes for each $k$.
More precisely, if we let $Z_i$ be the binary indicator of the event $\{ (k-1)/L \leq N_i/\log n < k/L \}$, then
$|\Y_k| = \sum_{i=1}^K Z_i$ 
% \al{
% \frac{|\Y_k|}{np_n} = \frac{1}{n p_n} \sum_{i=1}^K Z_i
% }
and Hoeffding's inequality implies that
\al{
\Pr\left( \left| |\Y_k| - E|\Y_k| \right| > \ep n p_n \right) \leq 2 e^{-2 n \ep^2 p_n^2},
}
for any $\ep > 0$.
If we define the event 
\al{
\E_k = \{ \left| |\Y_k| - E|\Y_k| \right| > \ep n p_n \},
}
we have
\al{
 H(\Y_k) & \leq H(\Y_k,\1_{\E_k}) \leq 1 + H(\Y_k | \1_{\E_k} ) \nonumber \\
 & \leq 1 + 2n \Pr(\E_k) + H(\Y_k | \bar \E_k ),
 \label{eq:bound1}
}
where we upper bound $H(\Y_k | \E_k)$ with $2n$, since $\Y$ can be fully described by a binary string of length $n$ and $n$ indicators of whether there is a cut at position $i$.

In order to bound $H(\Y_k | \bar \E_k )$, we first notice that the number of possible distinct sequences in $\Y_k$ is 
\aln{
\sum_{i=\frac{k-1}{L}\log n}^{\frac{k}{L}\log n} 2^i < 2 \cdot 2^{\frac{k}{L}\log n} = n^{k/L}.
}
Moreover, given $\bar \E_k$, 
\al{
 |\Y_k| & \leq E|\Y_k| + \ep n p_n  \nonumber \\
 & = np_n \left[ \ep + \Pr\left( \frac{k-1}{L} \leq \frac{N_1}{\log n} < \frac{k}{L}  \right) \right]
 = M,
 \label{eq:M}
}
and the set $\Y_k$ can be seen as a histogram $(x_1,...,x_{n^{k/L}})$ over all possible $n^{k/L}$  strings with $\sum x_i = M$.
Hence,
% The conditional entropy term in (\ref{eq:bound1}) can be bounded as
\al{
 H(\Y_k | \bar \E_k ) & \leq \log {{n^{k/L} + M -1}\choose{M}} \nonumber \\ 
 & \leq M \log \left(\frac{e(n^{k/L}+M-1)}{M} \right) \nonumber \\ 
 & = M \left[ \log \left(n^{k/L}+M-1\right) + \log(e) - \log M \right] \nonumber \\ 
& = M \left[ \max(\tfrac{k}{L}\log n,\log M) - \log M + o(\log n) \right] \nonumber \\
& = M \left[ (\tfrac{k}{L}\log n - \log M)^+ + o(\log n) \right] \nonumber \\
& = M \log n \left[ 
 (\tfrac{k}{L}  - \log M/\log n)^+ + o(1)
\right].
\label{eq:bound2}
}
From (\ref{eq:M}), we see that 
${\log M}/{\log n} \to 1$ as $n\to \infty$.
Combining (\ref{eq:bound1}) and (\ref{eq:bound2}), dividing by $n$ and letting $n \to \infty$ yields
\iscomment{$1+\ep$ missing below}
\al{
\lim_{n\to \infty} & \frac{H(\Y_k)}{n}
= \alpha \left( e^{-\alpha (k-1)/L} - e^{-\alpha k/L} \right) (\tfrac{k}{L} - 1)^+. 
}
Finally, we sum over $k$ to obtain
\iscomment{needs to deal with exchange of limit and sum below. maybe only sum up to some large but fixed value of k}
\al{
\lim_{n\to\infty} & \sum_{k=1}^\infty \frac{H(\Y_k)}{n} \nonumber \\
& = \sum_{k=L+1}^\infty \alpha \left( e^{-\alpha (k-1)/L} - e^{-\alpha k/L} \right) (\tfrac{k}{L} - 1) \nonumber \\
& = \frac{\alpha}{L} \sum_{k=L+1}^\infty  k \left( e^{-\alpha (k-1)/L} - e^{-\alpha k/L} \right) \nonumber \\
& \quad - \alpha \sum_{k=L+1}^\infty  \left( e^{-\alpha (k-1)/L} - e^{-\alpha k/L} \right) \nonumber \\
& = \frac{\alpha}{L} \sum_{k=L+1}^\infty  k \left( e^{-\alpha (k-1)/L} - e^{-\alpha k/L} \right) - \alpha e^{-\alpha}.
}
For the remaining summation, we obtain
\al{
\sum_{k=L+1}^\infty &  k \left( e^{-\alpha (k-1)/L} - e^{-\alpha k/L} \right) \nonumber \\
& = (L+1)e^{-\alpha} + \sum_{k=L+2}^\infty e^{-\alpha (k-1)/L} \nonumber \\
& = L e^{-\alpha} + e^{-\alpha} \sum_{k=0}^\infty e^{-\alpha k/L} \nonumber \\
& = L e^{-\alpha} + \frac{e^{-\alpha}}{1-e^{-\alpha/L}}.
}
We conclude that any achievable rate must satisfy
\al{
R & < \frac{\alpha}{L}  \left(Le^{-\alpha} + \frac{e^{-\alpha}}{1-e^{-\alpha/L}} \right) - \alpha e^{-\alpha} \nonumber \\
& = \frac{\alpha e^{-\alpha }}{L(1-e^{-\alpha/L})},
}
for any positive integer $L$.
Since 
\aln{
\lim_{L \to \infty} L(1-e^{-\alpha/L}) = \alpha,
}
we obtain the outer bound $R < e^{-\alpha}$.




\newpage 

We then have
\al{
H(\Y) & = H(\Y_1,...,\Y_n) \nonumber \\
& = H(\Y_1,...,\Y_n\left| |\Y_1|,...,|\Y_n| \right. ) + H( |\Y_1|,...,|\Y_n|  )  \nonumber  \\
&  \leq \sum_{k=1}^n H(\Y_k | |\Y_k|) + H( |\Y_1|,...,|\Y_n|  ).
}
Since $|\Y_k| \leq n$ for each $k$, a simple bound on $H( |\Y_1|,...,|\Y_n|  )$ is $\log n^2 = 2 \log n$.



Next we notice that conditioned on $|\Y_k| = m$, the set $\Y_k$ can be seen as a histogram $(x_1,...,x_{2^k})$ over all $2^k$ length-$k$ strings with $\sum x_i = m$.
Hence 
% \al{
%  H(\Y_k | |\Y_k| = m) & \leq \log {{2^k + m -1}\choose{m}} \nonumber \\ 
%  & \leq m \log \left(\frac{e(2^k+m-1)}{m} \right) \nonumber \\ 
% & = m \left[ k - \log m + o(1) \right], 
% }
\al{
 H(\Y_k | |\Y_k| = m) & \leq \log {{2^k + m -1}\choose{m}} \nonumber \\ 
 & \leq m \log \left(\frac{e(2^k+m-1)}{m} \right) \nonumber \\ 
 & = m \left[ \log \left(2^k+m-1\right) + \log(e) - \log m \right] \nonumber \\ 
& = m \left[ \max(k,\log m) - \log m + o(\log n) \right], \nonumber \\
& = m \left[ (k - \log m)^+ + o(\log n) \right].
}
Taking the expectation with respect to $m$, we obtain
\al{
& H (\Y_k | |\Y_k| ) \nonumber \\
& = \sum_{m=1}^{n} \Pr(|\Y_k| = m) m \left[ (k - \log m)^+ + o(\log n) \right] \nonumber \\ 
& = \sum_{m=1}^{2^k} \Pr(|\Y_k| = m) m \left[ k - \log m + o(\log n)  \right] \nonumber \\
& = E \left[ |\Y_k| \left[ k - \log |\Y_k| + o(\log n)  \right] | |\Y_k| \leq 2^k \right] \nonumber \\
& \quad \quad \quad \cdot \Pr(|\Y_k| \leq 2^k ) \nonumber \\
& = E \left[ |\Y_k| \left[ k - \log |\Y_k| + o(\log n)  \right] | |\Y_k| \leq 2^k \right] \nonumber \\
& \leq E \left[ |\Y_k|  |\Y_k| \leq 2^k \right] \left[ k - \log E \left[ |\Y_k|  |\Y_k| \leq 2^k \right] + o(\log n)  \right]   \nonumber \\
& \quad \quad \quad \cdot \Pr(|\Y_k| \leq 2^k ),
}
where the last step follows by applying Jensen's inequality to the concave function $g(x) = x(k-\log x)$.


\newpage

\iscomment{this needs to be explained}

Hence, for large $n$, we can view the $k$th channel as an instance of the shuffling channel \cite{DNAStorageISIT,noisyshuffling} with $E|\Y_k|$ fragments of length $(k/L)\log n$.
From the results in \cite{DNAStorageISIT}, the capacity of the $k$th channel is thus upper bounded by
\al{
& \lim_{n\to \infty}
\frac{E|\Y_k|\left[ (k/L) \log n - \log E|\Y_k| \right]}{E |\Y_k| (k/L) \log n} \nonumber \\
& = \lim_{n\to \infty}
1 - \frac{L \log E|\Y_k|}{k \log n} \nonumber \\
% }
% \al{
& = (1 - L/k)^+ = \left\{
\begin{array}{ll}
1 - L/k,  & \text{ for } k > L  \\
0 & \text{ for }k \leq L \\ 
\end{array}
% \begin{array}{ll}
% 1 - L/k, & \text{ for k > L} \\
% 0, & \text{ for k \leq L}
% \end{array}
\right.
}
where we used the fact that, from (\ref{eq:expyk}),
$\log E|\Y_k|/ \log n \to 1$ as $n \to \infty$.

In addition to Lemma~\ref{lem:exp1}, we will utilize a second result related to the asymptotic approximation of a geometric distribution as exponential.

\begin{lemma} \label{lem:exp2}
If $N^{(n)}$ is a ${\rm Geom}(p_n)$ random variable and $\lim_{n\to\infty} E[N^{(n)}]/\log n = \alpha$, then, for any $\beta \geq 0$,
\al{
\lim_{n \to \infty} & E\left[ N^{(n)} \1_{\{ N^{(n)} \geq \beta \log n  \}}\right] / \log n \nonumber \\
% \sum_{k=\beta \log n}^\infty & k \cdot \Pr( N^{(n)} = k )  =  \nonumber \\
& = E\left[ \tilde N \1_{\{ \tilde N \geq \beta   \}}\right]
= \left(\beta + \frac1\alpha\right)e^{-\alpha \beta},
}
where $\tilde N$ is an ${\rm Exponential}(\alpha)$ random variable.
\end{lemma}
Using Lemma~\ref{lem:exp2}, we can upper bound  the capacity achieved across all parallel channels as 
\al{
& \lim_{n\to\infty}  \sum_{k = 1}^\infty \frac{E|\Y_k| (k/L) \log n}{n}
\left(1-L/k\right)^+
\nonumber \\ 
& = \lim_{n\to\infty} \sum_{k = L+1}^\infty \frac{\alpha E|\Y_k| }{L n p_n}
\left(k-L\right) \\
& = \lim_{n\to\infty} \alpha \sum_{k = L+1}^\infty \frac{k}{L} \Pr\left( (k-1)/{L} \leq \tilde N_1 < k/L  \right)
 \nonumber \\
& \quad - \alpha \sum_{k = L+1}^\infty  e^{-\alpha (k-1)/L} - e^{-\alpha k/L}
\nonumber \\
& \approx \alpha E \left[ \tilde N_1 \1_{\{\tilde N_1 \geq 1\}} \right] - \alpha e^{-\alpha} \nonumber \\
& = \alpha \left( 1 + 1/\alpha \right)e^{-\alpha} - \alpha e^{-\alpha} = e^{-\alpha}.
}
\iscomment{several steps in the proof above need to be made more precise, especially the approximation step above (should depend on $L$)}


==> converse_04-09.tex <==
% !TEX root = main.tex


In order to prove the converse, we 
% view $\Y$ as a random set of strings (as opposed to an ordered list of strings).
first partition $\Y$ as $\cup_{k=1}^n \Y_k$, where
$\Y_k$ is the set of $k$-length strings in $\Y$.
Notice that $E|\Y| = np$ and $E|\Y_k| = q_i np$ where $q_k = (1-p)^k p$ is the probability that a ${\rm Geom}(p)$ random variable takes value $k$.
We then have
\al{
H(\Y) & = H(\Y_1,...,\Y_n) \nonumber \\
& = H(\Y_1,...,\Y_n\left| |\Y_1|,...,|\Y_n| \right. ) + H( |\Y_1|,...,|\Y_n|  )  \nonumber  \\
&  \leq \sum_{k=1}^n H(\Y_k | |\Y_k|) + H( |\Y_1|,...,|\Y_n|  ).
}
Since $|\Y_k| \leq n$ for each $k$, a simple bound on $H( |\Y_1|,...,|\Y_n|  )$ is $\log n^2 = 2 \log n$.
Next we notice that conditioned on $|\Y_k| = m$, the set $\Y_k$ can be seen as a histogram $(x_1,...,x_{2^k})$ over all $2^k$ length-$k$ strings with $\sum x_i = m$.
Hence 
\al{
 H(\Y_k | |\Y_k| = m) & \leq \log {{2^k + m -1}\choose{m}} \nonumber \\ 
 & \leq m \log \left(\frac{e(2^k+m-1)}{m} \right) \nonumber \\ 
& = m \left[ k - \log m + o(1) \right], 
}
and $H(\Y_k | |\Y_k|)  \leq E|\Y_k| \left[ k - \log E|\Y_k| + o(1) \right]$ by Jensen's inequality.
We conclude that 
\al{
\sum_{k=1}^n H(\Y_k | |\Y_k|) & \leq \sum_{k=1}^n q_k np \left[ k - \log (q_k np) + o(1) \right] \nonumber \\
& = n \left[ p E[{\rm Geom}(p)] - p H({\rm Geom}(p)) \right. \nonumber \\
& \quad \quad \quad \left. - p \log n + o(1) \right] \nonumber \\
& = n \left[ 1 - H(p) - p \log n + o(1) \right].
}
Using Fano's inequality, any achievable rate must be upper bounded by
\aln{
R \leq \frac{H(\Y)}{n} + \ep_n \leq 1 - H(p) - p \log n + o(1).
}
If $\lim_{n \to \infty} p \log n = \alpha < \infty$, then it must be the case that $p(n) \to 0$ as $n \to \infty$, which implies that $H(p) \to 0$ as $n \to \infty$, and $R \leq (1-\alpha)^+$.




==> converse_04-10.tex <==
% !TEX root = main.tex


In order to prove the converse, we 
% view $\Y$ as a random set of strings (as opposed to an ordered list of strings).
first partition $\Y$ as $\cup_{k=1}^n \Y_k$, where
$\Y_k$ is the set of $k$-length strings in $\Y$.
Notice that $E|\Y| = np$ and $E|\Y_k| = q_k np$ where $q_k = (1-p)^{k-1} p$ is the probability that a ${\rm Geom}(p)$ random variable takes value $k$.
We then have
\al{
H(\Y) & = H(\Y_1,...,\Y_n) \nonumber \\
& = H(\Y_1,...,\Y_n\left| |\Y_1|,...,|\Y_n| \right. ) + H( |\Y_1|,...,|\Y_n|  )  \nonumber  \\
&  \leq \sum_{k=1}^n H(\Y_k | |\Y_k|) + H( |\Y_1|,...,|\Y_n|  ).
}
Since $|\Y_k| \leq n$ for each $k$, a simple bound on $H( |\Y_1|,...,|\Y_n|  )$ is $\log n^2 = 2 \log n$.
Next we notice that conditioned on $|\Y_k| = m$, the set $\Y_k$ can be seen as a histogram $(x_1,...,x_{2^k})$ over all $2^k$ length-$k$ strings with $\sum x_i = m$.
Hence 
\al{
 H(\Y_k | |\Y_k| = m) & \leq \log {{2^k + m -1}\choose{m}} \nonumber \\ 
 & \leq m \log \left(\frac{e(2^k+m-1)}{m} \right) \nonumber \\ 
& = m \left[ k - \log m + o(1) \right], 
}
and $H(\Y_k | |\Y_k|)  \leq E|\Y_k| \left[ k - \log E|\Y_k| + o(1) \right]$ by Jensen's inequality.
We conclude that 
\al{
\sum_{k=1}^n H(\Y_k | |\Y_k|) & \leq \sum_{k=1}^n q_k np \left[ k - \log (q_k np) + o(1) \right] \nonumber \\
& = n \left[ p E[{\rm Geom}(p)] - p H({\rm Geom}(p)) \right. \nonumber \\
& \quad \quad \quad \left. - p \log n + o(1) \right] \nonumber \\
& = n \left[ 1 - H(p) - p \log n + o(1) \right].
}
Using Fano's inequality, any achievable rate must be upper bounded by
\aln{
R \leq \frac{H(\Y)}{n} + \ep_n \leq 1 - H(p) - p \log n + o(1).
}
If $\lim_{n \to \infty} p \log n = \alpha < \infty$, then it must be the case that $p_n \to 0$ as $n \to \infty$, which implies that $H(p) \to 0$ as $n \to \infty$, and $R \leq (1-\alpha)^+$.




==> converse_04-11.tex <==
% !TEX root = main.tex


In order to prove the converse, we 
% view $\Y$ as a random set of strings (as opposed to an ordered list of strings).
first partition $\Y$ as $\cup_{k=1}^n \Y_k$, where
$\Y_k$ is the set of $k$-length strings in $\Y$.
Notice that $E|\Y| = np$ and $E|\Y_k| = q_k np$ where $q_k = (1-p)^{k-1} p$ is the probability that a ${\rm Geom}(p)$ random variable takes value $k$.
We then have
\al{
H(\Y) & = H(\Y_1,...,\Y_n) \nonumber \\
& = H(\Y_1,...,\Y_n\left| |\Y_1|,...,|\Y_n| \right. ) + H( |\Y_1|,...,|\Y_n|  )  \nonumber  \\
&  \leq \sum_{k=1}^n H(\Y_k | |\Y_k|) + H( |\Y_1|,...,|\Y_n|  ).
}
Since $|\Y_k| \leq n$ for each $k$, a simple bound on $H( |\Y_1|,...,|\Y_n|  )$ is $\log n^2 = 2 \log n$.
Next we notice that conditioned on $|\Y_k| = m$, the set $\Y_k$ can be seen as a histogram $(x_1,...,x_{2^k})$ over all $2^k$ length-$k$ strings with $\sum x_i = m$.
Hence 
% \al{
%  H(\Y_k | |\Y_k| = m) & \leq \log {{2^k + m -1}\choose{m}} \nonumber \\ 
%  & \leq m \log \left(\frac{e(2^k+m-1)}{m} \right) \nonumber \\ 
% & = m \left[ k - \log m + o(1) \right], 
% }
\iscomment{update:}
\al{
 H(\Y_k | |\Y_k| = m) & \leq \log {{2^k + m -1}\choose{m}} \nonumber \\ 
 & \leq m \log \left(\frac{e(2^k+m-1)}{m} \right) \nonumber \\ 
 & = m \left[ \log \left(2^k+m-1\right) + \log(e) - \log m \right] \nonumber \\ 
& = m \left[ \max(k,\log m) - \log m + o(\log n) \right], \nonumber \\
& = m \left[ (k - \log m)^+ + o(\log n) \right].
}
Taking the expectation with respect to $m$, we obtain
\al{
& H (\Y_k | |\Y_k| ) \nonumber \\
& = \sum_{m=1}^{n} \Pr(|\Y_k| = m) m \left[ (k - \log m)^+ + o(\log n) \right] \nonumber \\ 
& = \sum_{m=1}^{2^k} \Pr(|\Y_k| = m) m \left[ k - \log m + o(\log n)  \right] \nonumber \\
& = E \left[ |\Y_k| \left[ k - \log |\Y_k| + o(\log n)  \right] | |\Y_k| \leq 2^k \right] \nonumber \\
& \quad \quad \quad \cdot \Pr(|\Y_k| \leq 2^k ) \nonumber \\
& = E \left[ |\Y_k| \left[ k - \log |\Y_k| + o(\log n)  \right] | |\Y_k| \leq 2^k \right] \nonumber \\
& \leq E \left[ |\Y_k|  |\Y_k| \leq 2^k \right] \left[ k - \log E \left[ |\Y_k|  |\Y_k| \leq 2^k \right] + o(\log n)  \right]   \nonumber \\
& \quad \quad \quad \cdot \Pr(|\Y_k| \leq 2^k ),
}
where the last step follows by applying Jensen's inequality to the concave function $g(x) = x(k-\log x)$.
Next we notice that 
\aln{
\sum_{k=1}^\infty k \cdot E \left[ |\Y_k|  |\Y_k| \leq 2^k \right]
}


\iscomment{still need to work on this}


and $H(\Y_k | |\Y_k|)  \leq E|\Y_k| \left[ k - \log E|\Y_k| + o(1) \right]$ by Jensen's inequality.
We conclude that 
\al{
\sum_{k=1}^n H(\Y_k | |\Y_k|) & \leq \sum_{k=1}^n q_k np \left[ k - \log (q_k np) + o(1) \right] \nonumber \\
& = n \left[ p E[{\rm Geom}(p)] - p H({\rm Geom}(p)) \right. \nonumber \\
& \quad \quad \quad \left. - p \log n + o(1) \right] \nonumber \\
& = n \left[ 1 - H(p) - p \log n + o(1) \right].
}
Using Fano's inequality, any achievable rate must be upper bounded by
\aln{
R \leq \frac{H(\Y)}{n} + \ep_n \leq 1 - H(p) - p \log n + o(1).
}
If $\lim_{n \to \infty} p \log n = \alpha < \infty$, then it must be the case that $p_n \to 0$ as $n \to \infty$, which implies that $H(p) \to 0$ as $n \to \infty$, and $R \leq (1-\alpha)^+$.




==> converse_05-14.tex <==
% !TEX root = main.tex

In order to prove the converse, we 
% view $\Y$ as a random set of strings (as opposed to an ordered list of strings).
first partition the input and output strings based on length.
% We consider a genie-aided approach to the converse, where encoder and decoder have knowledge of the tearing points $N_1,N_2,...$.
This allows us to view the torn-paper channel as a set of parallel channels, each of which involves fragments of roughly the same size.
%{\color{blue} can we complete this high-level description here? is it accurate to say we analyze each channel separately and then use concentration-type analysis to derive the outer-bound?}
More precisely, for an integer parameter $L$, we will let
% the $k$th channel will have input and output fragments given by
\al{
& \X_k = \left\{ \vX_i : \tfrac{k-1}{L} \log n \leq N_i < \tfrac{k}{L} \log n \right\}
\text{ and } \nonumber \\
& \Y_k = \left\{ \vY_i : \tfrac{k-1}{L} \log n \leq N_{\pi_i} < \tfrac{k}{L} \log n \right\},
\label{eq:ykdef}
}
for $k=1,2,...$,
and we will think of the transformation from $\X_k$ to $\Y_k$ as a separate channel.
% \iscomment{No actual transformation: $\X_k = \Y_k$}
Notice that the $k$th channel is intuitively similar to the shuffling channel with equal-length pieces considered in \cite{DNAStorageISIT}.
Also notice that 
% \iscomment{we may need to be a bit careful, because actually $E[K] = np - (1-p)$.}
% \al{
% E\left[|\Y_k|\right] & = E\left[ |\Y|\right] \Pr\left( \tfrac{k-1}{L} \log n \leq N_1 < \tfrac{k}{L} \log n \right) 
% \nonumber \\
% & = np_n \Pr\left( \frac{k-1}{L} \leq \frac{N_1}{\log n} < \frac{k}{L}  \right).
% \label{eq:expyk}
% }
\al{
E\left[|\Y_k|\right] 
& = E \left[ \sum_{i=1}^K \1  \left\{ \tfrac{k-1}{L} \log n \leq N_i < \tfrac{k}{L} \log n \right\} \right]
% & = E\left[ |\Y|\right] \Pr\left( \tfrac{k-1}{L} \log n \leq N_1 < \tfrac{k}{L} \log n \right) 
\nonumber \\
& = np_n \Pr\left( \frac{k-1}{L} \leq \frac{N_1}{\log n} < \frac{k}{L}  \right) + o(np_n).
\label{eq:expyk}
}
Notice that, since $\lim_{n\to\infty} p_n \log n = \alpha$, $E\left[\frac{N_1}{\log n}\right] \to \alpha^{-1}$ as $n \to \infty$.
Moreover, asymptotically, $\tilde N_1 = \frac{N_1}{\log n}$ approaches an ${\rm Exponential}(\alpha)$ random variable.
This known fact is stated as the following lemma, which we prove in Section~\ref{Section:appendix}.
% {\color{blue} can we cite a reference?}.
% \iscomment{removed $\Phi$ to shorten things}
\begin{lemma} \label{lem:exp1}
% Let $\Phi_{\alpha}(t) = e^{-\alpha t}$ be the complementary CDF of an ${\rm Exponential}(\alpha)$ random variable.
If $N^{(n)}$ is a ${\rm Geom}(p_n)$ random variable and $\lim_{n\to\infty} E[N^{(n)}]/\log n = 1/\alpha$, then
\al{
\lim_{n\to \infty}
\Pr\left( N^{(n)} \geq \beta \log n \right) = e^{-\alpha \beta}.
}
\end{lemma}
Using Lemma~\ref{lem:exp1} and (\ref{eq:expyk}),
we have that 
\al{
\lim_{n\to \infty} \frac{E\left[|\Y_k|\right]}{np_n} 
& = \lim_{n\to\infty} \Pr\left( \frac{k-1}{L} \leq \frac{N_1}{\log n} < \frac{k}{L}  \right) \nonumber \\
& = e^{-\alpha (k-1)/L} - e^{-\alpha k/L}.
}
\iflong
In addition, we will need a concentration inequality for $|\Y_k|$.
Notice that if we let $Z_i$ be the binary indicator of the event $\{ (k-1)/L \leq N_i/\log n < k/L \}$, then,
$|\Y_k| = \sum_{i=1}^K Z_i$.
However, since $K$ is also random, we cannot directly apply standard concentration inequalities. 
In Section~\ref{Section:appendix}, we prove the following lemma.
\else
In addition, the following lemma, proved in  Section~\ref{Section:appendix}, states that $|\Y_k|$ concentrates around its mean.
\fi
% \iscomment{should we just state lemmas as $\to 0$ as below?}
\begin{lemma} \label{lem:Ykconc}
% The number of fragments in $\Y_k$ satisfies
For any $\ep > 0$, 
as $n\to \infty$,
\al{
\Pr\left( \left| |\Y_k| - E|\Y_k| \right| > \ep n p_n \right)  
\to 0.
% 4 e^{-n p_n (\ep/2 - \ln (1+\ep/2))},
}
% for any $\ep > 0$.
\end{lemma}
If we define the event 
$\E_k = \{ \left| |\Y_k| - E|\Y_k| \right| > \ep n p_n \}$, then
\al{
 H(\Y_k) & \leq H(\Y_k,\1_{\E_k}) \leq 1 + H(\Y_k | \1_{\E_k} ) \nonumber \\
 & \leq 1 + 2n \Pr(\E_k) + H(\Y_k | \bar \E_k ) 
%  \nonumber \\
%  & 
%  = H(\Y_k | \bar \E_k ) +  o(n).
 \label{eq:bound1}
}
where we loosely upper bound $H(\Y_k | \E_k)$ with $2n$, since $\Y$ can be fully described by the binary string $X^n$ and $n-1$ indicators of the tearing points. 
% whether there is a cut at position $i$, for $i=1,...,n-1$.

In order to bound $H(\Y_k | \bar \E_k )$, \emph{i.e.}, the entropy of $\Y_k$ given that its size is close to the expected value, we first note that the number of possible distinct sequences in $\Y_k$ is 
\aln{
\sum_{i=\frac{k-1}{L}\log n}^{\frac{k}{L}\log n} 2^i < 2 \cdot 2^{\frac{k}{L}\log n} = 2n^{k/L}.
}
Moreover, given $\bar \E_k$,  \iscomment{$np_n$ issue}
\al{
 |\Y_k| & \leq E|\Y_k| + \ep n p_n  \nonumber \\
 & = np_n \left[ \ep + \Pr\left( \frac{k-1}{L} \leq \frac{N_1}{\log n} < \frac{k}{L}  \right) \right]
 \triangleq M,
 \label{eq:M}
}
and the set $\Y_k$ can be seen as a histogram $(x_1,...,x_{n^{k/L}})$ over all possible $n^{k/L}$  strings with $\sum x_i = M$.
Notice that we can view the last element of the histogram as containing ``excess counts'' if $|\Y_k| < M$.
Hence, from Lemma 1 in \cite{DNAStorageISIT},
% The conditional entropy term in (\ref{eq:bound1}) can be bounded as
\al{
 H(\Y_k | \bar \E_k ) & \leq \log {{2n^{k/L} + M -1}\choose{M}} \nonumber \\ 
 & \leq M \log \left(\frac{e(2n^{k/L}+M-1)}{M} \right) \nonumber \\ 
 & = M \left[ \log \left(2n^{k/L}+M-1\right) + \log(e) - \log M \right] \nonumber \\ 
& = M \left[ \max(\tfrac{k}{L}\log n,\log M) - \log M + o(\log n) \right] \nonumber \\
& = M \left[ (\tfrac{k}{L}\log n - \log M)^+ + o(\log n) \right] \nonumber \\
& = M \log n \left[ 
 (\tfrac{k}{L}  - \log M/\log n)^+ + o(1)
\right].
\label{eq:bound2}
}
From (\ref{eq:M}), we have
${\log M}/{\log n} \to 1$ as $n\to \infty$.
Combining (\ref{eq:bound1}) and (\ref{eq:bound2}), dividing by $n$, and letting $n \to \infty$ yields
\al{
\lim_{n\to \infty} & \frac{H(\Y_k)}{n}
= \lim_{n \to \infty} \frac{H(\Y_k|\bar \E_k) + 1 + 2n \Pr(\E_k)}{n}
\nonumber \\
& = \alpha \left( e^{-\alpha (k-1)/L} - e^{-\alpha k/L} + \ep \right) \left(\frac{k}{L} - 1\right)^+. 
\label{eq:limyk}
}
In order to bound an achievable rate $R$, we use Fano's inequality to obtain
\al{
n R & \leq I(X^n;\Y) + n \ep_n \leq H(\Y) + o(n), 
% \nonumber \\
% & = \sum_{k=1}^\infty H(\Y_k) + o(n), 
\label{eq:fano}
}
and we conclude that any achievable rate must satisfy
$
% R \leq \lim_{n\to \infty} \sum_{k=1}^\infty \frac{H(\Y_k)}{n}.
R \leq \lim_{n\to \infty} \frac{H(\Y)}{n}.
$
In order to connect (\ref{eq:fano}) and (\ref{eq:limyk}), we state the following lemma.
% \iscomment{maybe we don't need this lemma. could just sum over (12) before applying the limit.}
\begin{lemma} \label{lem:entropy}
If $\Y_k$ is defined as in (\ref{eq:ykdef}) for $k=1,...,\infty$,
\aln{
% \lim_{n\to \infty} \sum_{k=1}^\infty \frac{H(\Y_k)}{n} = 
\lim_{n\to \infty} \frac{H(\Y)}{n} \leq 
\sum_{k=1}^\infty \lim_{n\to \infty}  \frac{H(\Y_k)}{n}.
}
\end{lemma}
Based on this lemma, whose proof we provide in Section~\ref{Section:appendix}, we can upper bound any achievable rate $R$ by
\al{
R & \leq  \lim_{n\to\infty}   \frac{H(\Y)}{n} 
\leq \sum_{k=1}^\infty \lim_{n\to \infty}  \frac{H(\Y_k)}{n}
\nonumber \\
&
= \sum_{k=L+1}^\infty \alpha \left( e^{-\alpha (k-1)/L} - e^{-\alpha k/L} \right) (\tfrac{k}{L} - 1) \nonumber \\
& = \frac{\alpha}{L} \sum_{k=L+1}^\infty  k \left( e^{-\alpha (k-1)/L} - e^{-\alpha k/L} \right) \nonumber \\
& \quad - \alpha \sum_{k=L+1}^\infty  \left( e^{-\alpha (k-1)/L} - e^{-\alpha k/L} \right) \nonumber \\
& = \frac{\alpha}{L} \sum_{k=L+1}^\infty  k \left( e^{-\alpha (k-1)/L} - e^{-\alpha k/L} \right) - \alpha e^{-\alpha}.
}
For the remaining summation, we obtain
\al{
\sum_{k=L+1}^\infty &  k \left( e^{-\alpha (k-1)/L} - e^{-\alpha k/L} \right) \nonumber \\
& = (L+1)e^{-\alpha} + \sum_{k=L+2}^\infty e^{-\alpha (k-1)/L} \nonumber \\
& = L e^{-\alpha} + e^{-\alpha} \sum_{k=0}^\infty e^{-\alpha k/L} \nonumber \\
& = L e^{-\alpha} + \frac{e^{-\alpha}}{1-e^{-\alpha/L}}.
}
We conclude that any achievable rate must satisfy
\al{
R & < \frac{\alpha}{L}  \left(Le^{-\alpha} + \frac{e^{-\alpha}}{1-e^{-\alpha/L}} \right) - \alpha e^{-\alpha} \nonumber \\
& = \frac{\alpha e^{-\alpha }}{L(1-e^{-\alpha/L})},
}
for any positive integer $L$.
Since 
\aln{
\lim_{L \to \infty} L(1-e^{-\alpha/L}) = \alpha,
}
we obtain the outer bound $R < e^{-\alpha}$.



==> equivalence.tex <==
% !TEX root = main.tex

One of the challenges in proving Theorem~\ref{thm:capacity} is dealing with the fact that the total number of fragments $K$ is random.
Notice that, while we define $N_1,N_2,...$ to be i.i.d.~random variables, the fragment lengths $N_1,N_2,...,N_{K-1},n - \sum_{i=1}^{K-1} N_j$ are not independent.
In order to prove Theorem~\ref{thm:capacity}, we start by showing that the torn-paper channel described in Section~\ref{Section:Problem} has the same capacity as a similar channel where the total number of fragments is fixed at the expected number of fragments for the original channel.

More precisely, we consider a new channel whose input is again a length-$n$ binary string $X^n$, but the output is a set of $n p_n$ fragments.
We let $N_1,...,N_{n p_n}$ be i.i.d.~${\rm Geometric}(p_n)$ random variables and we let $X^* = (X_1,X_2,...)$ be an infinite sequence obtained by appending an infinite number of zeros to the right of $X^n$.
We then define $np_n$ fragments
\aln{
\vX_i = \left[X_{1+\sum_{j=1}^{i-1}{N_j}},...,X_{\sum_{j=1}^{i}{N_j}} \right],
}
for $i=1,...,n p_n$.
Just as in Section~\ref{Section:Problem}, we let the output strings be $Y_i = X_{T_i}$ for $i=1,...,np_n$, where $T_i$ is a permutation on $(1,...,n p_n)$, chosen uniformly at random.
Notice that the total length of the $Y$ strings is $\sum_{i=1}^{np_n} N_i$, which can take any positive value with positive probability.
We refer to this new channel as the \emph{unconstrained torn-paper channel} and let its capacity be $\Cunc$.
We then have the following channel equivalence.

\begin{lemma}
$C = \Cunc$.
\end{lemma}

\begin{proof}
We start by analyzing some aspects of the original torn-paper channel.
% Let $K$ be the number of fragments in the 
Notice that, if we let $T_i$, $i=2,...,n$, be binary variables indicating whether $X_i$ is the beginning of a fragment, then $T_2,...,T_n$ are i.i.d.~${\rm Bernoulli}(p)$ random variables and $K = 1 + \sum_{i=2}^n T_i$.
Therefore, 
\aln{
E[K] = 1 + (n-1)p_n = np_n + (1-p_n)
} 
and Hoeffding's inequality implies that 
% First we notice that 
% \al{
% | K - np_n | < \left| \sum_{i=1}^{np_n} N_i - n \right|
% \label{eq:Kbound}
% }
\al{
\Pr( & | K - np_n |  > \delta np_n ) \nonumber \\
& \leq \Pr( | K - E[K] | + (1-p_n) > \delta np_n  ) \nonumber \\
& \leq \Pr\left( | K - E[K] | > \delta n (p_n - n^{-1}(1-p_n) ) \right) \nonumber \\
% \leq \Pr \left( \left| \sum_{i=1}^{np_n} N_i - n \right| > \delta n p_n \right) \nonumber \\
% % & \leq \frac{{\rm Var}(N_1)}{\delta n p_n} = \frac{1-p_n}{\delta n p_n^3} = o(1),
% & \leq e^{-n p_n (\delta - \ln (1+\delta))}
% + e^{-n p_n (-\delta - \ln (1-\delta))} \nonumber \\
& \leq 2 e^{-2 n \delta^2 (p_n - n^{-1}(1-p_n) )^2} %\nonumber \\
%& 
\leq 2 e^{-n \delta^2},
\label{eq:Kconc}
}
where the last inequality holds for $n$ large enough.
% Intuitively this says that, for large $n$, $K \approx n p_n$, and the two channels are similar.

% We will prove that $C \leq \Cunc$ and $C \geq \Cunc$. 
We prove that $C \leq \Cunc$ first.
Consider a sequence of codes with rate $R$ and vanishing error probability for the original torn-paper channel.



\end{proof}

This result is unsurprising since, as $n \to \infty$, the torn-paper channel and this unconstrained version are nearly identical.
However, dealing with the unconstrained channel will simplify the achievability and converse of Theorem~\ref{thm:capacity} significantly.



==> interleaved.tex <==
% !TEX root = main.tex


While the scheme presented in Section~\ref{Section:Achievability} achieves the capacity of the torn-paper channel, it far from being a practical scheme.
In principle, it requires one to consider all possible $K!$ orderings of the $K$ fragments and trying to align each one to each of the $2^{nR}$ codewords.

A natural way to design schemes for a channel that shuffles fragments of the message involves placing ``indices'' on the different pieces, which allows properly ordering them.
However, as previously mentioned, the randomness in the tearing locations and in the length of the fragments makes this approach not straightforward.
In particular, if we place indices at evenly separated points of the input string $X^n$, they will appear at random locations of the fragments, and a fraction of the indices will be fragmented, making the recovery more difficult.
For that reason, in this section we explore the idea of \emph{interleaving} a pilot or synchronization sequence throughout the input codewords.

\begin{figure}[h] 
% 	\center
\vspace{-4mm}
\hspace{2mm}
       \includegraphics[width=0.85\linewidth]{interleave.pdf} 
      \caption{Interleaving a pilot sequence $\bp$ with message sequences
      $\bs_{u(1)},...,\bs_{u(m-1)}$ to form the codeword $\bc_u$.
      \label{fig:interleave} }
\end{figure}

The interleaving procedure to construct codewords is illustrated in Figure~\ref{fig:interleave}.
As we describe in more detail below, the pilot block $\bp$ and the message blocks $\bs_i$ are designed so that they have no string of length $\log n$ appears in both $\bp$ and $\bs_j$ for some $j$.
The ``sprinkled'' nature of the pilot sequence in $\bc_u$ prevents it from being fragmented by the tearing process.
More precisely, if we let $\beta n$ be the length of the pilot block $\bp$ and of each message block $\bs_j$, for $\beta \in (0,1)$, a fragment of length $N_i$ must contain at least $\beta N_i$ pilot symbols in it.
As we will see, provided that $N_i$ is long enough, this will allow its location on $X^n$ to be uniquely determined.


\subsection{Codeword construction}

For a fraction $\beta \in (0,1)$ to be determined later, we will construct a pilot sequence $\bp$ of length $\beta n$.
Notice that $\beta$ controls the fraction of the codeword that is dedicated to pilot symbols. 
The pilot sequence $\bp$ is constructed as a \emph{de Bruijn sequence} of order $\log (\beta n)$ \cite{debruijn}.
This sequence has length $2^{\log (\beta n)} = \beta n$ and it has the property that each length $\log (\beta n)$ substring appears exactly once.
A de Bruijn sequence of order $4$ is shown in Figure~\ref{fig:debruijn} for illustration.


Next we build a large set of message blocks $\S = \{\bs_1,...,\bs_M\}$, each of length $\beta n$, with the property that no length-2$\log(n)$ substring of $\bp$ appears in any of the message blocks.
Consider generating a binary sequence $\s$ with $\beta n$ symbols drawn as i.i.d.~${\rm Ber}(1/2)$ random variables.
The probability that a length-$k$ segment of the pilot $\bp$ appears in the random sequence $\s \in \F_2^{n/m}$ can be upper bounded as
\aln{
& \Pr\left( \bp[i:i+k-1] = \s[j:j+k-1], \right. \\ 
& \quad \quad \quad \left. \text{ for }\, 1 \leq i \leq \beta n - k, \; 1 \leq j \leq \beta n - k \right)  \\
& \quad \leq (\beta n)^2 2^{-k}
% = \left(\frac{n \, 2^{-k}}{m}\right)^{2}.
}
Therefore, if we let $k = (2+\delta) \log n$ for $\delta > 0$, %since $\ell = \tfrac12 \log \tfrac Gm \leq \tfrac12 \log G$, we obtain
\al{
& \Pr\left( \bp[i:i+k-1] = \s[j:j+k-1], \right. \nonumber \\
& \quad \quad \quad \left. \text{ for }\, 1 \leq i \leq n/m, \; 1 \leq j \leq n/m \right) 
\to 0, \label{alphaeq}
}
as $n \to \infty$.
%$\Pr\left( \s_i^k = \s_j^k, \, \text{ for }\, 0 \leq i < j \leq G-1 \right) \to 0$ as $G \to \infty$.
This means that for any $\ep > 0$, for $n$ large enough it is possible to choose $M = (1-\ep)2^{\beta n}$ sequences of length $\beta n$ that contain no length-$(2+\delta) \log n$ segment that is also in the pilot sequence $\bp$.
%can be concatenated with the pilot sequence to generate a length-$G$ sequence that has no repeats of length $\alpha \log G$.

Let $\S = \{\bs_1,...,\bs_{M}\}$ be a set with $M$ such sequences.
We build our actual code by taking $m-1$ sequences $\s_{i_1},...,\s_{i_{m-1}}$ from $\S$ and interleaving their symbols with the symbols from $\bp$.
More precisely, for each $u \in \{1,...,M\}^{m-1}$ we build the codeword $\bc_u = (c_u[0],...,c_u[n-1])$ as 
\aln{
c_u[mt + j] = \left\{ \begin{array}{l} p[t], \text{ for } j = 0, \; t = 0,...,n/m-1 \\
s_{u(j)}[t], \text{ for } j = 1,...,m-1, \; t = 0,...,n/m-1
\end{array}\right.
}
which is illustrated in Fig.~\ref{fig:interleave}.
%Each resulting codeword $\bc_i$ has the property that, for large enough $G$,
%\al{
%& (c_i[t],c_i[t+m],...,c_i[t+m \lfloor \alpha \log G \rfloor]) = (c_i[\tau],c_i[\tau+m],...,c_i[\tau+m \lfloor \alpha \log G \rfloor ]) \nonumber \\
%& \Longrightarrow \quad t \equiv \tau \bmod G. \label{norepeatseq}
%}
The resulting codebook $\C$ has $M^{m-1} = (1-\ep)^{\beta-1}2^{(1-\beta)n}$ codewords.






\subsection{Decoding and analysis}

\begin{itemize}
    \item suppose a random fragment has length $N_i > \frac2\beta \log n$
    \item then it will contain $ > 2 \log n$ pilot symbols in it
    \item it can only align to the codeword ``skeleton'' in a unique way
    \item so we recover all pieces that are longer than $\frac2\beta \log n$
    \item this gives us a coverage of 
    \aln{
    A(\beta) & = \frac{\sum_{k = \frac2\beta \log n}^\infty k (1-p)^{k-1}p}{1/p} \nonumber \\
    & = 
    1- \sum_{k=1}^{\frac2\beta \log n} k (1-p)^{k-1}p^2
    }
    \item the pieces lost are treated as erasures
    \item since a $\beta$-fraction of the sequence is used for the pilot sequence, we achieve a rate of
    \aln{
    \max_{\beta \in (0,1)} A(\beta) (1-\beta)
    }
    % \item we may be able to write $\lim_{n\to \infty} A(\beta)$ explicitly, since the the geometric distribution should be converging to an exponential distribution
    \item As $n \to \infty$, $E[N_i/\log n] \to {\rm Exp}(\alpha)$
    \item we can express $A(\beta)$ as
    \aln{
    A(\beta) & = \tfrac{\alpha}{\log n} E[N_i | N_i \geq \tfrac2\beta \log n] \Pr(N_i \geq \tfrac2\beta \log n) \\
    & = \alpha E[\tilde N_i | \tilde N_i \geq \tfrac2\beta] \Pr(\tilde N_i \geq \tfrac2\beta) \\
    & = \alpha( \tfrac{2}{\beta} + \tfrac1\alpha ) e^{-\tfrac{2\alpha}{\beta}}
    }
\end{itemize}


\newpage

\iscomment{The figure below if from an old draft. It needs to be adapted for this case.}



\begin{figure}[h] 
	\center
       \includegraphics[width=0.75\linewidth]{align.pdf} 
       \caption{Aligning a read $\r$ incorrectly to the generic codeword $\bc_?$.\label{alignfig} }
\end{figure}





==> related_work.tex <==

\vspace{2mm}
\noindent {\bf Related literature:}
The problem of reconstructing a string from a set of its subsequences has been studied in 
% different contexts, such as the 
the context of the
assembly problem \cite{MotahariDNA,BBT}, the trace reconstruction problem \cite{holenstein2008trace,srinivasavaradhan2018maximum,cheraghchi2019coded}, and the problem of reconstructing a string from its substring spectrum \cite{gabrys2018unique,marcovich2019reconstruction}.
% We point out that, i
In all of these settings, the set of observed strings have overlaps with each other, which is different from the case considered here.

\iflong
Several recent works have designed codes tailored to specific aspects of DNA storage.
% based on this general model, some of which were implemented in proof-of-concept storage systems \cite{church_next-generation_2012,goldman_towards_2013,grass_robust_2015,bornholt_dna-based_2016,erlich_dna_2016}. 
% Several papers have studied important additional aspects of the design of a practical DNA storage system.
These include DNA synthesis constraints such as sequence composition  \cite{kiah_codes_2016,yazdi_rewritable_2015,erlich_dna_2016}, the asymmetric nature of the DNA sequencing error channel \cite{gabrys_asymmetric_2015}, 
the need for codes that correct insertion errors \cite{sala_insertions_2016}, 
and the need for techniques to allow random access \cite{yazdi_rewritable_2015}.
% The use of fountain codes for DNA storage was considered in both \cite{erlich_dna_2016} and \cite{mackay_near-capacity_2015}. 
% Finally, the recent paper~\cite{lenz_upper_2019} studies a related channel and proves a converse on the capacity through a combination of techniques, including ideas from~\cite{DNAStorageISIT,noisyshuffling}.
\fi

Motivated by DNA-based storage, a few recent works have considered the problem of coding across an unordered set of strings 
\cite{DNAStorageISIT,LenzAnchor,lenz2018coding} and the problem of coding over sets  \cite{kovavcevic2018codes,song2018sequence}.
\iflong
Channels that shuffle blocks of information were also recently studied in the context of the \emph{bee-identification problem} \cite{tandon2019bee} and noisy permutation channels \cite{makur2018information}.
\fi
% ILAN: For the journal version, we should cite and look at lele wang's work on de Bruijn seq for synchronization \cite{wang2017quickest}

